Deep Active Learning for Regression Using $\epsilon$-weighted Hybrid Query Strategy

Designing an inexpensive approximate surrogate model that captures the salient features of an expensive high-fidelity behavior is a prevalent approach in design optimization. In recent times, Deep Learning (DL) models are being used as a promising surrogate computational model for engineering problems. However, the main challenge in creating a DL-based surrogate is to simulate/label a large number of design points, which is time-consuming for computationally costly and/or high-dimensional engineering problems. In the present work, we propose a novel sampling technique by combining the active learning (AL) method with DL. We call this method $\epsilon$-weighted hybrid query strategy ($\epsilon$-HQS) , which focuses on the evaluation of the surrogate at each learning iteration and provides an estimate of the failure probability of the surrogate in the Design Space. By reusing already collected training and test data, the learned failure probability guides the next iteration's sampling process to the region of the high probability of failure. During the empirical evaluation, better accuracy of the surrogate was observed in comparison to other methods of sample selection. We empirically evaluated this method in two different engineering design domains, finite element based static stress analysis of submarine pressure vessel(computationally costly process) and second submarine propeller design( high dimensional problem). https://github.com/vardhah/epsilon_weighted_Hybrid_Query_Strategy

==> 1.Introduction.tex <==
\section{Introduction}
\label{sec:introduction}



%Design problems in engineering and scientific community is an ongoing challenge and in most cases these design problems are in high dimension with exponential large number of choices and includes complex relationship between design parameters. Design space exploration is a process to understand the effect of design variables on the performance metrics and analyse the complex relationship between these variables on the performance metrics.  
%The process usually involves successive sampling in the design space and analyse the performance metric to find promising design point or subspace which satisfy all the constraints and meet the necessary performance requirement. Learning these nonlinear hyper-planes about the relationship between input design variables and performance metrics is the  role of human design engineer. For this purpose design engineer evaluate/simulate the design space at various samples and try to create a response surface in his mind. This response surface is further used in future to find the design for a given performance metrics.  

However the process has multiple issues: first, without any strategic sampling approach, the trivial randomized sampling approach to generate data  becomes unavailing in high dimension design variable space because the number of points needed to give reasonably uniform coverage rises exponentially- this phenomenon is infamously called the curse of dimensionality. Another issue is related to the simulation models and the simulation process has an iterative subroutine and consequently long simulation time. Due to these reasons in most practical problems, design engineers always search for optimal design near already explored region of design space. 
%Accordingly, produced design is locally optimal and may be sub-optimal over all possible designs.  
Alternative is to freeze many of the design variables at hopefully meaningful values and work with just a few at a time, iterating around to understand the impact of various variable progressively. Both these issues do not resolve the problem of efficient global exploration. The Utopian solution would be is to learn the hyper-plane with few number of strategic samples(fewer iterative simulation cycles) and learned model should have capability to parallelise the evaluation process on modern hardware(GPU).  Machine learning and specially Deep Learning perfectly fit in this scenario. Learning these hyperplane using Deep learning models which can interpolate  can assist human designer to find good design in highly complex nonlinear relationship.

For a given design space with known boundaries, the goal here is to create a data driven DL based surrogate model for the simulation process. The benefit of the creating a surrogate is parallel faster evaluation of design points, which can speed up the whole design decision process.  However there are many questions that need to answered before creating a data-driven surrogate in real design space, which are:
\begin{enumerate}
    \item What would be the step-size of sampling? : There is no existing approach to find the meaningful step-size without knowledge of the hyperplane. Selection of step size of sampling will be crucial for accuracy of reproduction of result by surrogate. 
  
    \item How should we sample to generate data? As randomized sampling  is not feasible and may soon reach to exponential size.
\end{enumerate}

In most of the problem setting, we rely on Theories for data modeling which often assume that the data are provided by a source that we do not control, but we can active sample from the data source. However, for most practical problem there are two complex situation which needs attention.  First, when data measurements/evaluation are relatively expensive or slow and in such case we want to know where to sample so as to learn as maximum as possible, and second, when there is an immense amount of data and we want to select a subset of data that maximise my trained model performance. Both these scenarios needs a objectively estimating the utility of candidate data points. Active learning framework directly address the estimation of utility of candidate data points.  On other hand Deep Learning model has powerful learning capability, and can scale to high dimension data and automatically extract feature in large dimensional problems. By combining DL with AL,called DeepAL we can retain strong learning capability of DL while getting benefited from strategic samples selected by AL. Although AL related-research on query strategy is quite rich, its direct application in DL framework is difficult. The underlying reason is: 
\begin{enumerate}
    \item Lack of uncertainty in prediction: Uncertainty-based Query strategy is important direction in AL. Deep Learning framework does not give uncertainty directly. Researchers has addressed this problem by two alternative approaches: either by using  models that can estimate uncertainty directly, such as Bayesian Neural network, or by ensembling models to estimate uncertainty indirectly. Bayesian methods become expensive when number of samples in thousands or input dimension is greater than 10. Ensemble-methods require independent training of several models, which is also time consuming.  
    
    \item Most AL framework works on single sample per iteration , while in DL framework, retaining neural network after each single datapoint is not computationally feasible.
    
\end{enumerate}

 
Compared with the multiple research work on Deep active learning for classification, there are only a few approaches for Deep active learning for regression problem. For classification problem, its is probability of class, which can be easily used with other statistical measure (like Shannon's Entropy function) to create a query strategy. Many research work has leveraged it and create one or other flavour of query strategy.However the problem under study in this paper is regression, for which model's prediction is a scalar value. In such case direct statistical measure cannot be deployed. To counter this researchers took the route of Bayesian framework to measure variance in estimation by ensemble the predictors. 


In conclusion, our approach differs from other randomised sampling methods and can certainly be
used for sampling in large design space for creation of surrogate model.  Specifically, this technique:
\begin{itemize}
    \item provides a feedback mechanism for selecting strategic samples during design space exploration and can help to learn the input-output behaviour of a function/simulator in less number of evaluations. 
    \item verifies the performance gains from this novel approach in terms of lesser number of evaluation and better accuracy in comparison to other sampling methods.

\end{itemize}

The remainder of this paper is organized as follows: Section 2 formally defines a problem statement . In Section 3, we describe our methodology in details. In Section 4 we present our experiments and will evaluate the results. Section 5 discusses related work. We will conclude in Section 6 with a brief discussion of future work.




